Safe learning-based optimal motion planning for automated driving

This paper presents preliminary work on learning the search heuristic for the optimal motion planning for automated driving in urban traffic. Previous work considered search-based optimal motion planning framework (SBOMP) that utilized numerical or model-based heuristics that did not consider dynamic obstacles. Optimal solution was still guaranteed since dynamic obstacles can only increase the cost. However, significant variations in the search efficiency are observed depending whether dynamic obstacles are present or not. This paper introduces machine learning (ML) based heuristic that takes into account dynamic obstacles, thus adding to the performance consistency for achieving real-time implementation.

==> macros/packages.tex <==
%============================================================================
% The following packages can be found on http:\\www.ctan.org
% BIBTEX
%\usepackage{cite}
% BIBLATEX: \usepackage[style=IEEEtran,backend=bibtex]{biblatex}

\usepackage{graphicx}  % for pdf, bitmapped graphics files
\usepackage{array}
%\usepackage{epsfig}   % for postscript graphics files
%\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times}     % assumes new font selection scheme installed
\usepackage[fleqn]{amsmath}   % assumes amsmath package installed
\usepackage{amssymb}   % assumes amsmath package installed
%\usepackage{mathabx}   % for \widebar % Böse (font 3)
\usepackage{dsfont}
\usepackage{float}     % for placing with (H) at a specific position 
\usepackage{textgreek}
\usepackage[table]{xcolor}  % Färbige Tabellen
\usepackage{booktabs}       % Schöne Tabellen (dicke und dünne Linien)
\usepackage{filemod}        % für autoupdate bei geänderten tikz-grafiken
\usepackage{xifthen}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{epstopdf}
\usepackage{subcaption}
\usepackage{paralist}
\usepackage{footnote}
%==============================================================================
% macro for executing a shell command immidiatly 
%\newcommand{\runmycommand}[1]{\immediate\write18{#1}}
% AUTOMATIC BIBTEX
\IfFileExists{\jobname.aux}% needs --enable-write18
             {\typeout{bibtex \jobname.aux}
              \immediate\write18{bibtex \jobname.aux}
              \typeout{*** AUTO RUNNING BIBTEX ***}}
             {\typeout{*********** Rerun for bibliography *************}}
%FOR BIBLATEX %\addbibresource{./IEEEabrv,./library}
             
% Pakete für Blockdiagramme und Diagramme
\usepackage{tikz}               % Achtung die Reihenfolge der Tikz Pakete ist
\usepackage{pgfplots}           % entscheidend!
\usepackage{pgfplotstable} 
\usepgfplotslibrary{groupplots}
\usepgfplotslibrary{units}
%\usetikzlibrary{spy}
\usetikzlibrary{shadows,positioning,arrows}
%\usetikzlibrary{shapes,shapes.multipart}
\usetikzlibrary{calc}
\usetikzlibrary{trees,fit,backgrounds}
%\usetikzlibrary{patterns,decorations.pathreplacing,decorations.pathmorphing}
%\usetikzlibrary{decorations.markings}
\usetikzlibrary{matrix}
\usetikzlibrary{shadows.blur,shapes.symbols}

%=================================================================================
\usepgfplotslibrary{external} % PDFs machen
\tikzexternalize[prefix=tikz_temp/]     % Unterordner für PDFs
\newcommand\autoupdateexternfigure[2]{  % MAKRO UM AUTOUPDATE ZU ERMÖGLICHEN
  \tikzsetnextfilename{#2}              % pdf-filename
  \filemodCmp{#1}{tikz_temp/#2.log}%    % prüft file datum 
  {\tikzset{external/force remake=true}}% erzwingt remake wenn log alt
  {}
}
%\tikzset{external/force remake} % immer alle Bilder neu machen
% Achtung für später: EPS-Grafiken können mit Tikz auch automatisch erstellt werden (siehe Internet)
% Tipps zu eps: auf http://tex.stackexchange.com/questions/8641/export-eps-figures-from-tikz
%=================================================================================

% Spezial Worttrennungen
\hyphenation{Last-rampen Betriebs-punkt}

%============================================================================
% PDF-Einstellungen
%\usepackage[ pdfauthor={Zlatan Ajanovic, Michael Stolz, Martin Horn}
%             ,pdftitle={A Novel Observer Concept for Embedded Drivetrain Applications}
%             ,pdfpagelayout=TwoPageLeft
%             ,pdfstartview  = {FitV}
%             %,pdfpagemode  = UseAttachments %OPEN ATTACHMENTS-VIEW IN PD
%             ,pdfpagelabels = true
%             ,linkcolor     = {black}
%             ,colorlinks    = {true} 
%             ,citecolor     = {black}
%             ,urlcolor      = {black}
%             ,bookmarks, bookmarksnumbered
%             %,bookmarksopen={true}, 
%             %,pagebackref  = true, backref = page     %% turn on backreferencing
%             ,plainpages    = false
%             ,hypertexnames = true
%             ]{hyperref}
%============================================================================
% Matrizen ------------------------------------------------------------------  
%\usepackage{arydshln}         % have dotted lines to separate matrix elements 
%\newcommand{\myhdots}{\hdashline[.4pt/1.5pt]}          % macro für punktierte

==> macros/tikzStyles.tex <==
\tikzstyle{s} = [font = \footnotesize]

\tikzstyle{doppelpfeil} = [-latex,postaction={draw,shorten >=6pt,-latex}]
\tikzstyle{sarrowtip} = [>=latex]  
\tikzstyle{myarrowtip} = [>=implies] 

\tikzset{curveinscope/.style={every path/.style={draw=white, double distance=1pt, line width=2pt, double=black, text=black}}}

\DeclareRobustCommand{\myLine}[1]{
(\tikzset{external/export next=false}\begin{tikzpicture}%
\useasboundingbox (-0.2ex,0) rectangle (4.65ex,1ex);%
\draw[line width=0.3ex,#1](0,0.65ex)--(4.5ex,0.65ex);%
\end{tikzpicture})}



